RoutePlacer: An End-to-End Routability-Aware Placer with Graph Neural Network

Placement is a critical and challenging step of modern chip design, with routability being an essential indicator of placement quality. Current routability-oriented placers typically apply an iterative two-stage approach, wherein the first stage generates a placement solution, and the second stage provides non-differentiable routing results to heuristically improve the solution quality. This method hinders jointly optimizing the routability aspect during placement. To address this problem, this work introduces RoutePlacer, an end-to-end routability-aware placement method. It trains RouteGNN, a customized graph neural network, to efficiently and accurately predict routability by capturing and fusing geometric and topological representations of placements. Well-trained RouteGNN then serves as a differentiable approximation of routability, enabling end-to-end gradient-based routability optimization. In addition, RouteGNN can improve two-stage placers as a plug-and-play alternative to external routers. Our experiments on DREAMPlace, an open-source AI4EDA platform, show that RoutePlacer can reduce Total Overflow by up to 16% while maintaining routed wirelength, compared to the state-of-the-art; integrating RouteGNN within two-stage placers leads to a 44% reduction in Total Overflow without compromising wirelength.

==> chapters/a_1_ablation.tex <==
\section{Ablation Study}
\label{sec:app-abla}
We further analyze how our method optimizes routability. We compared our gradient which generates by our method(ours.w.o. inflat) with the original DREAMPlace without the routability-driven method (DREAMPlace.w.o. inflat) and the result is shown in Table \ref{tab:noinflat-dac2012} and \ref{tab:noinflat-ispd2011}. We can see that: Compared with the original DREAMPlace using gradient to optimize routability can improve 16\% in total overflow. This demonstrates that the topological structure plays a vital role in routability optimization. Incorporating with topological structure can aid in identifying narrow areas and potential congestion cells and spread them out to reduce overall overflow

We also further visualize the placement and show the distribution of overflow on grid cells in Fig \ref{fig:sb14-hist-noinflat} and \ref{fig:sb10-hist-noinflat}. We can see that on \texttt{superblue} and \texttt{superblue}, compared with the original DREAMPlace, using the gradient to optimize routability shows fewer grid cell numbers on each overflow level, especially in high overflow level, which displays the performance of topological structure optimization on narrow area.

\begin{figure}[htbp]
	\includegraphics[width=70mm]{figure/visualization/ablation/noinflat/superblue14_hist.png}
	\caption{Comparsion of routing grid cell overflow statistic between DREAMPlace and ours.w.o. inflat on \texttt{superblue14} from \texttt{DAC2012}.}
	\label{fig:sb14-hist-noinflat}
\end{figure}

\begin{figure}[htbp]
	\includegraphics[width=70mm]{figure/visualization/ablation/noinflat/superblue10_hist.png}
	\caption{Comparsion of routing grid cell overflow statistic between DREAMPlace and ours.w.o. inflat on \texttt{superblue10} from \texttt{ISPD2011}.}
	\label{fig:sb10-hist-noinflat}
\end{figure}

\begin{table*}[]
	\caption{Ablation experiments on \texttt{DAC2012}. Ours.w.o.inflat represents cell inflation not integrated. DREAMPlace is version 1.0 without a routability-driven method.}
	\label{tab:noinflat-dac2012}
	\resizebox{1.0\linewidth}{!}{
	\begin{tabular}{lcc|cc|cc|cc|cc|cc}
		\hline
		\multirow{2}{*}{Netlist} & \multirow{2}{*}{\#cell} & \multirow{2}{*}{\#nets} & \multicolumn{2}{c|}{TOF} & \multicolumn{2}{c|}{MOF} & \multicolumn{2}{c|}{H-CR} & \multicolumn{2}{c|}{V-CR} & \multicolumn{2}{c}{WL} \\ 
		\cline{4-13} 
		& & & Ours.w.o.inflat & DREAMPlace.w.o.inflat & Ours.w.o.inflat & DREAMPlace.w.o.inflat & Ours.w.o.inflat & DREAMPlace.w.o.inflat & Ours.w.o.inflat & DREAMPlace.w.o.inflat & Ours.w.o.inflat & DREAMPlace.w.o.inflat \\ 
		\hline
		superblue2 & 1014K & 991K & 1153398 & \textbf{1152128} & 56 & \textbf{54} & 0.56 & \textbf{0.52} & \textbf{0.27} & 0.32 & 22.83 & \textbf{22.82} \\
		superblue3 & 920K & 898K & \textbf{236218} & 240382 & 64 & \textbf{52} & 0.64 & \textbf{0.52} & \textbf{0.23} & 0.27 & 14.29 & \textbf{14.25} \\
		superblue6 & 1014K & 1007K & \textbf{132370} & 205802 & 52 & \textbf{48} & 0.51 & \textbf{0.5} & \textbf{0.22} & 0.24 & \textbf{14.33} & 14.37 \\
		superblue7 & 1365K & 1340K & \textbf{21198} & 22050 & \textbf{16} & 20 & 0.2 & \textbf{0.19} & \textbf{0.15} & 0.18 & 19.21 & \textbf{19.19} \\
		superblue11 & 955K & 936K & \textbf{46704} & 79720 & 16 & 16 & 0.22 & 0.22 & \textbf{0.12} & 0.13 & \textbf{14.36} & 14.42 \\
		superblue12 & 1293K & 1293K & 2112070 & \textbf{1478142} & 104 & \textbf{90} & 0.8 & \textbf{0.71} & 0.45 & \textbf{0.41} & 15.47 & \textbf{15.02} \\
		superblue14 & 635K & 620K & \textbf{20482} & 23490 & 24 & \textbf{20} & \textbf{0.3} & 0.25 & 0.13 & \textbf{0.12} & 9.89 & \textbf{9.88} \\
		superblue16 & 699K & 697K & \textbf{23776} & 24110 & 24 & 24 & \textbf{0.26} & 0.28 & \textbf{0.18} & 0.19 & 10.47 & \textbf{10.46} \\
		superblue19 & 523K & 512K & \textbf{61098} & 82312 & \textbf{32} & 40 & 0.34 & 0.4 & \textbf{0.18} & 0.22 & \textbf{6.72} & 6.81 \\
		\multicolumn{3}{l|}{Average ratio} & 1.00 & 1.17 & 1.00 & 0.99 & 1.00 & 0.96 & 1.00 & 1.09 & 1.00 & 1 \\ 
		\hline
	\end{tabular}
}
\end{table*}


\begin{table*}[]
	\caption{Ablation experiments on \texttt{ISPD2011}.}
	\label{tab:noinflat-ispd2011}
	\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{lcc|cc|cc|cc|cc|cc}
			\toprule
			\multirow{2}{*}{Netlist} & \multirow{2}{*}{\#cell} & \multirow{2}{*}{\#nets} & \multicolumn{2}{c|}{TOF} & \multicolumn{2}{c|}{MOF} & \multicolumn{2}{c|}{H-CR} & \multicolumn{2}{c|}{V-CR} & \multicolumn{2}{c}{WL} \\ 
			\cmidrule{4-13} 
			& & & Ours.w.o.inflat & DREAMPlace.w.o.inflat & Ours.w.o.inflat & DREAMPlace.w.o.inflat & Ours.w.o.inflat & DREAMPlace.w.o.inflat & Ours.w.o.inflat & DREAMPlace.w.o.inflat & Ours.w.o.inflat & DREAMPlace.w.o.inflat \\ 
			\midrule
			superblue1 & 848K & 823K & \textbf{72380} & 74694 & \textbf{16} & 20 & 0.22 & 0.22 & \textbf{0.19} & 0.2 & \textbf{12.9} & 12.91 \\
			superblue2 & 1014K & 991K & \textbf{709172} & 895270 & 46 & 40 & 0.54 & 0.51 & \textbf{0.26} & 0.31 & \textbf{25.19} & 25.29 \\
			superblue4 & 600K & 568K & \textbf{114232} & 119732 & \textbf{36} & 44 & \textbf{0.45} & 0.53 & \textbf{0.21} & 0.25 & \textbf{9.18} & 9.19 \\
			superblue5 & 773K & 787K & \textbf{348976} & 363260 & \textbf{32} & 34 & 0.43 & 0.43 & 0.26 & 0.24 & \textbf{15.31} & 15.36 \\
			superblue10 & 1129K & 1086K & \textbf{142986} & 251602 & 20 & 20 & 0.29 & 0.28 & \textbf{0.15} & 0.16 & \textbf{24.1} & 24.33 \\
			superblue12 & 1293K & 1293K & \textbf{2112070} & 2201282 & \textbf{104} & 112 & \textbf{1.13} & 1.22 & 0.59 & 0.55 & \textbf{15.47} & 15.56 \\
			superblue15 & 1124K & 1080K & \textbf{115962} & 116112 & 16 & 16 & \textbf{0.25} & 0.26 & 0.13 & 0.13 & \textbf{14.51} & 14.52 \\
			superblue18 & 484K & 469K & \textbf{100336} & 104162 & 16 & 16 & \textbf{0.25} & 0.27 & 0.19 & 0.18 & \textbf{8.65} & 8.67 \\
			\multicolumn{3}{l|}{Average ratio} & 1.00 & 1.15 & 1.00 & 1.06 & 1.00 & 1.04 & 1.00 & 1.04 & 1.00 & 1.01 \\ 
			\bottomrule
		\end{tabular}
	}
\end{table*}

==> chapters/rebuttal.tex <==
\section{Explanation of the method's effectiveness}
\label{sec:app-effect}

Our method optimizes routability when generating placement, giving it an edge over traditional two-stage methods, wherein solution generation is agnostic of routability. Traditional placers optimize Half-Perimeter Wirelength and overlaps without considering routing, leading to congestion issues. Optimizing congestion faces two main challenges: (1) Routing is only available post-placement, and (2) It’s hard to differentiate routing results like congestion and optimize them with gradient-based optimizers. Our solution involves training a GNN as a differentiable estimation of congestion, allowing us to (1) predict congestion in placement, and (2) use gradients of predicted congestion for gradient-based optimization.
